Efficient Use of Spectral Resources in Wireless Communication Using Training Data Optimization

Wireless communication applications has acquired a vastly increasing range over the past decade. This rapidly increasing demand implies limitations on utilizing wireless resources. One of the most important resources in wireless communication is frequency spectrum. This thesis provides different solutions towards increasing the spectral efficiency. The first solution provided in this thesis is to use a more accurate optimization metric: maximal acheivable rate (compared to traditional metric: ergodic capacity) to optimize training data size in wireless communication. Training data symbols are previously known symbols to the receiver inserted in data packets which are used by receiver to acquire channel state information (CSI). Optimizing training data size with respect to our proposed tight optimization metric, we could achieve higher rates especially for short packet and ultra reliable applications. Our second proposed solution to increase spectral efficiency is to design a multifunction communication and sensing platform utilizing a special training sequence design. We proposed a platform where two training sequences are designed, one for the base-station and the other for the user. By designing these two training sequence such that they are uncorrelated to each other, the base station will be able to distinguish between the two training sequence. Having one of the sequences especially designed for radar purposes (by designing it such that it has an impulse-like autocorrelation), the system will be able to sense the environment, transmit and receive the communication data simultaneously.

==> Packages.tex <==
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage[font=footnotesize]{subfig}
\usepackage[font=small]{caption}
\usepackage[percent]{overpic} 
%\usepackage{cite}	% interfering with format a
\usepackage{array}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\usepackage{color,soul}
\usepackage{hyperref}
\usepackage{framed}
\usepackage{amsmath}
\usepackage{amsfonts}

\usepackage{dsfont}

%%%%%%%%%%%%%%%%%%%%%%%%%% My own Packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{float} % for floating figures [H]
\RequirePackage{longtable}
\usepackage{algorithm}
\usepackage{tabularx}
\usepackage{longtable}
\usepackage{ltxtable}

%%%%%%%%%%%%%%%%%%%%%%%%%% My own Packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\TODO}[1]{{\color{red}{\textbf{\hl{#1}}}}}
\newcommand{\ignore}[1]{}

\DeclareMathOperator*{\argmin}{argmin}

%\renewcommand{\baselinestretch}{1}		For single spacing :)


\usepackage[final]{pdfpages}

\newcommand{\myPart}[3]{
\vspace{25cm}
\begin{minipage}{0.8\linewidth}
\begin{center}
\end{center}
\end{minipage}

\vspace{#3}
\begin{center}
{\fontsize{2cm}{4.5cm}\selectfont Part  #1}
\end{center}

\vspace{1.0cm}
\begin{center}
{\fontsize{2cm}{4.5cm}\selectfont #2}
\end{center}
}

\newcommand{\myCopyRight}[3]{
\begin{center}

\noindent\fbox{
\begin{minipage}{{#3}\textwidth}
\vspace{-2mm}
\begin{singlespace}
\emph{Parts of this chapter have been presented in #1. Copyright \textcircled{c} #2, IEEE.} 
\end{singlespace} 
\vspace{2mm}
\end{minipage}
\vspace{20pt}
}
\end{center}
}

\newcommand{\myCopyRightSpringer}[3]{

\noindent\begin{center}

\noindent\fbox{
\begin{minipage}{{#3}\textwidth}
\vspace{-2mm}
\begin{singlespace}
\emph{Parts of this chapter have been presented in #1. Copyright \textcircled{c} #2, Springer.} 
\end{singlespace} 
\vspace{2mm}
\end{minipage}
\vspace{20pt}
}
\end{center}
}

\newif\ifiThenticate

\newcommand{\RemoveIFiThenticate}[1]{
\ifiThenticate
\else
#1
\fi
}

\iThenticatefalse



